On the Effectiveness of Automated Metrics for Text Generation Systems

A major challenge in the field of Text Generation is evaluation because we lack a sound theory that can be leveraged to extract guidelines for evaluation campaigns. In this work, we propose a first step towards such a theory that incorporates different sources of uncertainty, such as imperfect automated metrics and insufficiently sized test sets. The theory has practical applications, such as determining the number of samples needed to reliably distinguish the performance of a set of Text Generation systems in a given setting. We showcase the application of the theory on the WMT 21 and Spot-The-Bot evaluation data and outline how it can be leveraged to improve the evaluation protocol regarding the reliability, robustness, and significance of the evaluation outcome.

==> tables/alpha60_rho90_eta90_fixed.tex <==
\begin{tabular}{ c | c  c c c c c }
    \multicolumn{ 7}{c}{$|\mathcal{T_M}|$} \\ \hline
    %\multirow{ 11 }{*}{\STAB{\rotatebox[origin=c]{90}{$  |\mathcal{T_O}|$}}}
      & 0  & $1e^3$  &  $5e^3$  & $1e^4$  & $5e^4$  & $1e^5$  \\ \hline
    
         0  & 1.000  & 0.054   & 0.024  & 0.017  & 0.008  & 0.005  \\
    
         10  & 0.379  & 0.054    & 0.024  & 0.017  & 0.008  & 0.005  \\
    
         50  & 0.187  & 0.052    & 0.024  & 0.017  & 0.008  & 0.005  \\
    
         100  & 0.134  & 0.050    & 0.024  & 0.017  & 0.008  & 0.005  \\
    
         250  & 0.085  & 0.046   & 0.023  & 0.017  & 0.008  & 0.005  \\
    
         500  & 0.061  & 0.040    & 0.022  & 0.016  & 0.008  & 0.005  \\
    
          $1e^3$  & 0.043  & 0.034    & 0.021  & 0.016  & 0.008  & 0.005  \\
    
         $2.5e^3$  & 0.027  & 0.024   & 0.018  & 0.014  & 0.007  & 0.005  \\
    
          $5e^3$  & 0.019  & 0.018   & 0.015  & 0.013  & 0.007  & 0.005  \\
    
          $1e^4$  & 0.014  & 0.013    & 0.012  & 0.011  & 0.007  & 0.005  \\
    
\end{tabular}


==> tables/eps1.tex <==

\begin{tabular}{c | c | c c c c c c c c c c c c c c}
    \multicolumn{16}{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{15}{*}{\STAB{\rotatebox[origin=c]{90}{$|\mathcal{T_{\rho, \eta}}| = |\mathcal{T_O}|$}}}
    &          & $128$ & $256$ & $512$ & $1024$ & $2048$ & $4096$ & $8192$ & $2^{14}$ & $2^{15}$ & $2^{16}$ &  $2^{17}$ & $2^{18}$ & $2^{19}$ & $2^{20}$ \\ \hline
    & $128$     & 0.114  & 0.113  & 0.112  & 0.111  & 0.110  & 0.110  & 0.110  & 0.110  & 0.110  & 0.110  & 0.110  & 0.110  & 0.110  & 0.110  \\
    & $256$     & 0.082  & 0.081  & 0.080  & 0.079  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  \\
    & $512$     & 0.059  & 0.058  & 0.058  & 0.057  & 0.056  & 0.056  & 0.055  & 0.055  & 0.055  & 0.055  & 0.055  & 0.055  & 0.055  & 0.055  \\
    & $1024$     & 0.042  & 0.042  & 0.041  & 0.041  & 0.040  & 0.040  & 0.039  & 0.039  & 0.039  & 0.039  & 0.039  & 0.039  & 0.039  & 0.039  \\
    & $2048$     & 0.030  & 0.030  & 0.030  & 0.029  & 0.029  & 0.028  & 0.028  & 0.028  & 0.028  & 0.028  & 0.028  & 0.028  & 0.028  & 0.028  \\
    & $4096$     & 0.021  & 0.021  & 0.021  & 0.021  & 0.021  & 0.020  & 0.020  & 0.020  & 0.020  & 0.020  & 0.020  & 0.020  & 0.020  & 0.020  \\
    & $8192$     & 0.015  & 0.015  & 0.015  & 0.015  & 0.015  & 0.015  & 0.014  & 0.014  & 0.014  & 0.014  & 0.014  & 0.014  & 0.014  & 0.014  \\
    & $2^{14}$     & 0.011  & 0.011  & 0.011  & 0.011  & 0.011  & 0.010  & 0.010  & 0.010  & 0.010  & 0.010  & 0.010  & 0.010  & 0.010  & 0.010  \\
    & $2^{15}$     & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  \\
    & $2^{16}$     & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  \\
    & $2^{17}$     & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.003  \\
    & $2^{18}$     & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.002  \\
    & $2^{19}$     & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  \\
    & $2^{20}$     & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  \\
\end{tabular}

%\rotatebox[origin=c]{90}{rota}}

==> tables/eps2.tex <==
\label{tab:alpha60_rho90_eta90}
\begin{tabular}{c | c | c c c c c c c c c c c c c c}
    \multicolumn{16}{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{15}{*}{\STAB{\rotatebox[origin=c]{90}{$|\mathcal{T_{\rho, \eta}}| = |\mathcal{T_O}|$}}}
    &          & $128$ & $256$ & $512$ & $1024$ & $2048$ & $4096$ & $8192$ & $2^{14}$ & $2^{15}$ & $2^{16}$ &  $2^{17}$ & $2^{18}$ & $2^{19}$ & $2^{20}$ \\ \hline
    & $128$     & 0.101  & 0.094  & 0.088  & 0.084  & 0.081  & 0.080  & 0.079  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  & 0.078  \\
    & $256$     & 0.076  & 0.071  & 0.066  & 0.061  & 0.058  & 0.056  & 0.055  & 0.054  & 0.054  & 0.054  & 0.054  & 0.054  & 0.054  & 0.054  \\
    & $512$     & 0.056  & 0.053  & 0.050  & 0.046  & 0.043  & 0.040  & 0.039  & 0.038  & 0.037  & 0.037  & 0.037  & 0.037  & 0.037  & 0.037  \\
    & $1024$     & 0.041  & 0.040  & 0.038  & 0.035  & 0.032  & 0.030  & 0.028  & 0.027  & 0.027  & 0.026  & 0.026  & 0.026  & 0.026  & 0.026  \\
    & $2048$     & 0.029  & 0.029  & 0.028  & 0.027  & 0.025  & 0.023  & 0.021  & 0.020  & 0.019  & 0.019  & 0.019  & 0.018  & 0.018  & 0.018  \\
    & $4096$     & 0.021  & 0.021  & 0.020  & 0.020  & 0.019  & 0.018  & 0.016  & 0.015  & 0.014  & 0.014  & 0.013  & 0.013  & 0.013  & 0.013  \\
    & $8192$     & 0.015  & 0.015  & 0.015  & 0.014  & 0.014  & 0.013  & 0.012  & 0.011  & 0.011  & 0.010  & 0.010  & 0.009  & 0.009  & 0.009  \\
    & $2^{14}$     & 0.011  & 0.011  & 0.011  & 0.010  & 0.010  & 0.010  & 0.009  & 0.009  & 0.008  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  \\
    & $2^{15}$     & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.007  & 0.006  & 0.006  & 0.005  & 0.005  & 0.005  & 0.005  \\
    & $2^{16}$     & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.005  & 0.004  & 0.004  & 0.004  & 0.004  & 0.003  \\
    & $2^{17}$     & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.004  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  \\
    & $2^{18}$     & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.003  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  \\
    & $2^{19}$     & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.002  & 0.001  \\
    & $2^{20}$     & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  & 0.001  \\
\end{tabular}

==> tables/showcase1/bleurt-20-ref-C_no100_nm0.tex <==
\begin{tabular}{ c | c c c }
     & FBAI ( 0.67 )   & VT ( 0.65 )   & HT ( 0.58 )   \\ \hline
    
        FBAI ( 0.67 )  & -  & 0.02 (0.615)  & 0.09 (0.904)  \\
    
        VT ( 0.65 )  & -0.02 (0.382)  & -  & 0.07 (0.843)  \\
    
        HT ( 0.58 )  & -0.09 (0.095)  & -0.07 (0.155)  & -  \\
    
\end{tabular}


==> tables/showcase1/bleurt-20-ref-C_no100_nm1000.tex <==
\begin{tabular}{ c | c c c }
     & FBAI ( 0.66 )   & VT ( 0.62 )   & HT ( 0.56 )   \\ \hline
    
        FBAI ( 0.66 )  & -  & 0.04 (0.742)  & 0.09 (0.933)  \\
    
        VT ( 0.62 )  & -0.04 (0.256)  & -  & 0.05 (0.801)  \\
    
        HT ( 0.56 )  & -0.09 (0.066)  & -0.05 (0.197)  & -  \\
    
\end{tabular}


==> tables/showcase1/bleurt-20-ref-C_no527_nm0.tex <==
\begin{tabular}{ c | c c c }
     & FBAI ( 0.67 )   & VT ( 0.64 )   & HT ( 0.58 )   \\ \hline
    
        FBAI ( 0.67 )  & -  & 0.02 (0.798)  & 0.09 (0.998)  \\
    
        VT ( 0.64 )  & -0.02 (0.197)  & -  & 0.06 (0.978)  \\
    
        HT ( 0.58 )  & -0.09 (0.002)  & -0.06 (0.021)  & -  \\
    
\end{tabular}


==> tables/showcase1/bleurt_theoretical.tex <==
\begin{tabular}{ c | c | c c c }
    \multicolumn{ 5 }{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{ 5 }{*}{\STAB{\rotatebox[origin=c]{90}{$  |\mathcal{T_O}|$}}}
    &  & 0  & 1000  & 10000  \\ \hline
    
        & 0  & 1.000  & 0.413  & 0.354  \\
    
        & 50  & 0.183  & 0.165  & 0.158  \\
    
        & 100  & 0.131  & 0.123  & 0.120  \\
    
        & 527  & 0.057  & 0.057  & 0.056  \\
    
\end{tabular}


==> tables/showcase1/sentBLEU-ref-C_no100_nm0.tex <==
\begin{tabular}{ c | c c c }
     & FBAI ( 0.67 )   & VT ( 0.65 )   & HT ( 0.58 )   \\ \hline
    
        FBAI ( 0.67 )  & -  & 0.02 (0.615)  & 0.09 (0.904)  \\
    
        VT ( 0.65 )  & -0.02 (0.382)  & -  & 0.07 (0.843)  \\
    
        HT ( 0.58 )  & -0.09 (0.095)  & -0.07 (0.155)  & -  \\
    
\end{tabular}


==> tables/showcase1/sentBLEU-ref-C_no100_nm1000.tex <==
\begin{tabular}{ c | c c c }
     & FBAI ( 0.67 )   & VT ( 0.64 )   & HT ( 0.57 )   \\ \hline
    
        FBAI ( 0.67 )  & -  & 0.02 (0.631)  & 0.09 (0.918)  \\
    
        VT ( 0.64 )  & -0.02 (0.366)  & -  & 0.07 (0.854)  \\
    
        HT ( 0.57 )  & -0.09 (0.081)  & -0.07 (0.144)  & -  \\
    
\end{tabular}


==> tables/showcase1/sentBLEU-ref-C_no527_nm0.tex <==
\begin{tabular}{ c | c c c }
     & FBAI ( 0.67 )   & VT ( 0.64 )   & HT ( 0.58 )   \\ \hline
    
        FBAI ( 0.67 )  & -  & 0.02 (0.798)  & 0.09 (0.998)  \\
    
        VT ( 0.64 )  & -0.02 (0.197)  & -  & 0.06 (0.978)  \\
    
        HT ( 0.58 )  & -0.09 (0.002)  & -0.06 (0.021)  & -  \\
    
\end{tabular}


==> tables/showcase1/sentbleu_full_test.tex <==
\begin{tabular}{ l | c c  }
\multicolumn{ 3 }{c}{$|\mathcal{T_O}| = 527, |\mathcal{T_M}| = 0$} \\ \hline
$\pi(\alpha_1) - \pi(\alpha_2)$   & $\epsilon$   & $P(\alpha_1 > \alpha_2)$   \\ \hline
FBAI(0.67) - VT (0.64)  & 0.02  & 0.798   \\
FBAI(0.67) - HT (0.58)  & 0.09  & 0.998  \\
VT(0.64) - HT (0.58)    & 0.06  & 0.978  \\\hline
\multicolumn{ 3 }{c}{$|\mathcal{T_O}| = 100, |\mathcal{T_M}| = 0$} \\ \hline
$\pi(\alpha_1) - \pi(\alpha_2)$   & $\epsilon$   & $P(\alpha_1 > \alpha_2)$   \\ \hline
FBAI(0.67) - VT (0.65)  & 0.02  & 0.615   \\
FBAI(0.67) - HT (0.58)  & 0.09  & 0.904  \\
VT(0.65) - HT (0.58)    & 0.07  & 0.843  \\\hline
\multicolumn{ 3 }{c}{$|\mathcal{T_O}| = 100, |\mathcal{T_M}| = 1000$} \\ \hline
$\pi(\alpha_1) - \pi(\alpha_2)$   & $\epsilon$   & $P(\alpha_1 > \alpha_2)$   \\ \hline
FBAI(0.66) - VT (0.62)  & 0.04  & 0.742   \\
FBAI(0.66) - HT (0.56)  & 0.09  & 0.933  \\
VT(0.62) - HT (0.56)    & 0.05  & 0.801  \\\hline
\end{tabular}


==> tables/showcase1/sentbleu_theoretical.tex <==
\begin{tabular}{ c | c | c c c }
    \multicolumn{ 5 }{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{ 5 }{*}{\STAB{\rotatebox[origin=c]{90}{$  |\mathcal{T_O}|$}}}
    &  & 0  & 1000  & 10000  \\ \hline
    
        & 0  & 1.000  & 0.754  & 0.741  \\
    
        & 50  & 0.183  & 0.181  & 0.181  \\
    
        & 100  & 0.131  & 0.130  & 0.129  \\
    
        & 527  & 0.057  & 0.057  & 0.057  \\
    
\end{tabular}


==> tables/showcase2/better_theoretical.tex <==
\begin{tabular}{ c | c | c c c }
    \multicolumn{ 5 }{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{ 5 }{*}{\STAB{\rotatebox[origin=c]{90}{$  |\mathcal{T_O}|$}}}
    &  & 0  & 1000  & 10000  \\ \hline
    
        & 0  & 1.000  & 0.067  & 0.044  \\
    
        & 50  & 0.176  & 0.062  & 0.043  \\
    
        & 100  & 0.126  & 0.059  & 0.042  \\
    
        & 600  & 0.052  & 0.041  & 0.033  \\
    
\end{tabular}


==> tables/showcase2/usr_ret_no100_nm0.tex <==
\begin{tabular}{ c | c c c }
     & BL ( 0.38 )   & LiC ( 0.30 )   & KV ( 0.25 )   \\ \hline
    
        BL ( 0.38 )  & -  & 0.08 (0.882)  & 0.14 (0.983)  \\
    
        LiC ( 0.30 )  & -0.08 (0.117)  & -  & 0.06 (0.827)  \\
    
        KV ( 0.25 )  & -0.14 (0.016)  & -0.06 (0.170)  & -  \\
    
\end{tabular}


==> tables/showcase2/usr_ret_no100_nm10000.tex <==
\begin{tabular}{ c | c c c }
     & BL ( 0.36 )   & LiC ( 0.28 )   & KV ( 0.22 )   \\ \hline
    
        BL ( 0.36 )  & -  & 0.08 (0.889)  & 0.13 (0.989)  \\
    
        LiC ( 0.28 )  & -0.08 (0.109)  & -  & 0.06 (0.851)  \\
    
        KV ( 0.22 )  & -0.13 (0.010)  & -0.06 (0.147)  & -  \\
    
\end{tabular}


==> tables/showcase2/usr_ret_no600_nm0.tex <==
\begin{tabular}{ c | c c c }
     & BL ( 0.38 )   & LiC ( 0.30 )   & KV ( 0.24 )   \\ \hline
    
        BL ( 0.38 )  & -  & 0.08 (0.999)  & 0.13 (1.000)  \\
    
        LiC ( 0.30 )  & -0.08 (0.001)  & -  & 0.06 (0.989)  \\
    
        KV ( 0.24 )  & -0.13 (0.000)  & -0.06 (0.010)  & -  \\
    
\end{tabular}


==> tables/showcase2/usr_theoretical.tex <==
\begin{tabular}{ c | c | c c c }
    \multicolumn{ 5 }{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{ 5 }{*}{\STAB{\rotatebox[origin=c]{90}{$  |\mathcal{T_O}|$}}}
    &  & 0  & 1000  & 10000  \\ \hline
    
        & 0  & 1.000  & 0.751  & 0.735  \\
    
        & 50  & 0.176  & 0.174  & 0.173  \\
    
        & 100  & 0.126  & 0.125  & 0.124  \\
    
        & 600  & 0.052  & 0.052  & 0.052  \\
    
\end{tabular}


==> tables/spot_the_bot/pairwise_reduced_full_oracle.tex <==
\begin{tabular}{ c | c c c c c c c }
     & BL  & LiC   & KV  \\ \hline
BL  & -  & 0.08 (0.999)  & 0.13 (1.000)  \\
LiC  & -0.08 (0.001)  & -  & 0.06 (0.989)  \\
KV  &  -0.13 (0.000)  & -0.06 (0.010)  & -  \\
\end{tabular}


==> tables/spot_the_bot/stb_pairwise_additional.tex <==
\begin{tabular}{ c | c c c c c c }
     & BL   & LiC   & KV   & HF   & BR   & S2S   \\ \hline
    
        BL  & -  & 0.08 (0.999)  & 0.13 (1.000)  & 0.20 (1.000)  & 0.31 (1.000)  & 0.33 (1.000)  \\
    
        LiC  & -0.08 (0.001)  & -  & 0.06 (0.991)  & 0.12 (1.000)  & 0.23 (1.000)  & 0.25 (1.000)  \\
    
        KV  & -0.13 (0.000)  & -0.06 (0.009)  & -  & 0.07 (0.999)  & 0.17 (1.000)  & 0.20 (1.000)  \\
    
        HF  & -0.20 (0.000)  & -0.12 (0.000)  & -0.07 (0.001)  & -  & 0.11 (1.000)  & 0.13 (1.000)  \\
    
        BR  & -0.31 (0.000)  & -0.23 (0.000)  & -0.17 (0.000)  & -0.11 (0.000)  & -  & 0.02 (0.965)  \\
    
        S2S  & -0.33 (0.000)  & -0.25 (0.000)  & -0.20 (0.000)  & -0.13 (0.000)  & -0.02 (0.032)  & -  \\
    
\end{tabular}


==> tables/spot_the_bot/stb_pairwise_matched.tex <==
\begin{tabular}{ c | c c c c c c }
     & BL   & LiC   & KV   & HF   & BR   & S2S   \\ \hline
    
        BL  & -  & 0.08 (0.999)  & 0.13 (1.000)  & 0.20 (1.000)  & 0.31 (1.000)  & 0.34 (1.000)  \\
    
        LiC  & -0.08 (0.001)  & -  & 0.06 (0.990)  & 0.12 (1.000)  & 0.23 (1.000)  & 0.26 (1.000)  \\
    
        KV  & -0.13 (0.000)  & -0.06 (0.010)  & -  & 0.07 (0.998)  & 0.18 (1.000)  & 0.20 (1.000)  \\
    
        HF  & -0.20 (0.000)  & -0.12 (0.000)  & -0.07 (0.001)  & -  & 0.11 (1.000)  & 0.14 (1.000)  \\
    
        BR  & -0.31 (0.000)  & -0.23 (0.000)  & -0.18 (0.000)  & -0.11 (0.000)  & -  & 0.02 (0.974)  \\
    
        S2S  & -0.34 (0.000)  & -0.26 (0.000)  & -0.20 (0.000)  & -0.14 (0.000)  & -0.02 (0.024)  & -  \\
    
\end{tabular}


==> tables/spot_the_bot/stb_pairwise_oracle.tex <==
\begin{tabular}{ c | c c c c c c }
     & BL   & LiC   & KV   & HF   & BR   & S2S   \\ \hline
    
        BL  & -  & 0.08 (0.999)  & 0.13 (1.000)  & 0.20 (1.000)  & 0.31 (1.000)  & 0.34 (1.000)  \\
    
        LiC  & -0.08 (0.001)  & -  & 0.06 (0.989)  & 0.12 (1.000)  & 0.23 (1.000)  & 0.26 (1.000)  \\
    
        KV  & -0.13 (0.000)  & -0.06 (0.010)  & -  & 0.07 (0.998)  & 0.18 (1.000)  & 0.20 (1.000)  \\
    
        HF  & -0.20 (0.000)  & -0.12 (0.000)  & -0.07 (0.002)  & -  & 0.11 (1.000)  & 0.14 (1.000)  \\
    
        BR  & -0.31 (0.000)  & -0.23 (0.000)  & -0.18 (0.000)  & -0.11 (0.000)  & -  & 0.02 (0.974)  \\
    
        S2S  & -0.34 (0.000)  & -0.26 (0.000)  & -0.20 (0.000)  & -0.14 (0.000)  & -0.02 (0.024)  & -  \\
    
\end{tabular}


==> tables/spot_the_bot/theoretical_bounds.tex <==
\begin{tabular}{ c | c | c c c c c }
    \multicolumn{ 6 }{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{ 5 }{*}{\STAB{\rotatebox[origin=c]{90}{$|\mathcal{T_O}|$}}}
    &  & 0  & 1000  &  10000  & 100000  \\ \hline
    
    & 0  & 1.000  & 0.734   & 0.733   & 0.733  \\

    & 100  & 0.134  & 0.124  & 0.123   & 0.123  \\
    
    & 250  & 0.085  & 0.080   & 0.079   & 0.079  \\
    
    & 500  & 0.061  & 0.057   & 0.056   & 0.056  \\
\end{tabular}

==> tables/wmt21/pairwise_reduced_full_oracle.tex <==
\begin{tabular}{ c | c c c c c c c }
     & FBAI  & VT   & HT  \\ \hline
        FBAI  & -  & 0.03 (0.842)  & 0.09 (0.998)  \\
       VT  & -0.03 (0.154)  & -  & 0.06 (0.974)  \\
        HT  & -0.09 (0.001)  & -0.06 (0.025)  & -  \\
\end{tabular}


==> tables/wmt21/theoretical_bounds.tex <==
\begin{tabular}{ c | c | c c c c c }
    \multicolumn{ 6 }{c}{$|\mathcal{T_M}|$} \\ \hline
    \multirow{ 5 }{*}{\STAB{\rotatebox[origin=c]{90}{$|\mathcal{T_O}|$}}}
    &  & 0  & 1000  &  10000  & 100000  \\ \hline
    
    & 0  & 1.000  & 0.734   & 0.733   & 0.733  \\

    & 100  & 0.134  & 0.124  & 0.123   & 0.123  \\
    
    & 250  & 0.085  & 0.080   & 0.079   & 0.079  \\
    
    & 500  & 0.061  & 0.057   & 0.056   & 0.056  \\
\end{tabular}

==> tables/wmt21/wmt21_pairwise_both.tex <==
\begin{tabular}{ c | c c c c c c c }
     & Facebook-AI   & VolcTrans-GLAT   & Online-W   & Nemo   & VolcTrans-AT   & UEdin   & HuaweiTSC   \\ \hline
    
        Facebook-AI  & -  & 0.03 (0.842)  & 0.03 (0.881)  & 0.04 (0.905)  & 0.06 (0.980)  & 0.08 (0.998)  & 0.09 (0.998)  \\
    
        VolcTrans-GLAT  & -0.03 (0.154)  & -  & 0.01 (0.568)  & 0.01 (0.611)  & 0.03 (0.849)  & 0.05 (0.966)  & 0.06 (0.974)  \\
    
        Online-W  & -0.03 (0.116)  & -0.01 (0.425)  & -  & 0.00 (0.539)  & 0.02 (0.802)  & 0.05 (0.950)  & 0.05 (0.961)  \\
    
        Nemo  & -0.04 (0.092)  & -0.01 (0.382)  & -0.00 (0.454)  & -  & 0.02 (0.776)  & 0.05 (0.942)  & 0.05 (0.955)  \\
    
        VolcTrans-AT  & -0.06 (0.019)  & -0.03 (0.147)  & -0.02 (0.194)  & -0.02 (0.219)  & -  & 0.02 (0.789)  & 0.03 (0.822)  \\
    
        UEdin  & -0.08 (0.002)  & -0.05 (0.033)  & -0.05 (0.049)  & -0.05 (0.056)  & -0.02 (0.206)  & -  & 0.00 (0.543)  \\
    
        HuaweiTSC  & -0.09 (0.001)  & -0.06 (0.025)  & -0.05 (0.038)  & -0.05 (0.043)  & -0.03 (0.173)  & -0.00 (0.450)  & -  \\
    
\end{tabular}


==> tables/wmt21/wmt21_pairwise_oracle.tex <==
\begin{tabular}{ c | c c c c c c c }
     & Facebook-AI   & VolcTrans-GLAT   & Online-W   & Nemo   & VolcTrans-AT   & UEdin   & HuaweiTSC   \\ \hline
    
        Facebook-AI  & -  & 0.02 (0.798)  & 0.03 (0.848)  & 0.03 (0.862)  & 0.05 (0.968)  & 0.08 (0.997)  & 0.09 (0.998)  \\
    
        VolcTrans-GLAT  & -0.02 (0.197)  & -  & 0.01 (0.573)  & 0.01 (0.598)  & 0.03 (0.844)  & 0.06 (0.971)  & 0.06 (0.978)  \\
    
        Online-W  & -0.03 (0.148)  & -0.01 (0.420)  & -  & 0.00 (0.522)  & 0.02 (0.794)  & 0.05 (0.955)  & 0.05 (0.966)  \\
    
        Nemo  & -0.03 (0.134)  & -0.01 (0.395)  & -0.00 (0.471)  & -  & 0.02 (0.775)  & 0.05 (0.949)  & 0.05 (0.961)  \\
    
        VolcTrans-AT  & -0.05 (0.031)  & -0.03 (0.152)  & -0.02 (0.202)  & -0.02 (0.220)  & -  & 0.03 (0.808)  & 0.03 (0.840)  \\
    
        UEdin  & -0.08 (0.003)  & -0.06 (0.028)  & -0.05 (0.043)  & -0.05 (0.049)  & -0.03 (0.187)  & -  & 0.00 (0.546)  \\
    
        HuaweiTSC  & -0.09 (0.002)  & -0.06 (0.021)  & -0.05 (0.033)  & -0.05 (0.038)  & -0.03 (0.156)  & -0.00 (0.447)  & -  \\
    
\end{tabular}

